The Large High Altitude Air Shower Observatory (LHAASO) Science Book (2021 Edition)

Since the science white paper of the Large High Altitude Air Shower Observatory (LHAASO) published on arXiv in 2019 [e-Print: 1905.02773 (astro-ph.HE)], LHAASO has completed the transition from a project to an operational gamma-ray astronomical observatory LHAASO is a new generation multi-component facility located in Daocheng, Sichuan province of China, at an altitude of 4410 meters. It aims at measuring with unprecedented sensitivity the spectrum, composition, and anisotropy of cosmic rays in the energy range between 10$^{12}$ and 10$^{18}$~eV, and acting simultaneously as a wide aperture (one stereoradiant) continuously operating gamma-ray telescope in the energy range between 10$^{11}$ and $10^{15}$~eV with the designed sensitivity of 1.3\% of the Crab Unit (CU) above 100 TeV. LHAASO's capability of measuring simultaneously different shower components (electrons, muons, and Cherenkov/fluorescence light), will allow it to investigate the origin, acceleration, and propagation of CR through measurement of the energy spectrum, elemental composition, and anisotropy with unprecedented resolution. The remarkable sensitivity of LHAASO will play a key role in CR physics and gamma-ray astronomy for a general and comprehensive exploration of the high energy universe and will allow important studies of fundamental physics (such as indirect dark matter search, Lorentz invariance violation, quantum gravity) and solar and heliospheric physics. The LHAASO Collaboration organized an editorial working group and finished all editorial work of this science book, to summarize the instrumental features and outline the prospects of scientific researches with the LHAASO experiment.

==> ENDA-Detector.tex <==
\subsection{Contribution of ENDA to LHAASO}
\subsubsection{Motivation}

When arriving at Earth, high energy cosmic rays interact with the air nuclei originating extensive air showers (EAS). 
They consist of a core of high energy hadrons that continuously feed the electromagnetic part of the shower, mainly with photons from neutral pion, kaon and eta particle decays. Nucleons and other high energy hadrons contribute to the hadronic cascade. 
High energy hadrons, which constitute the EAS skeleton, may carry important information for multi-parameter correlation studies, since some hadronic observables, primarily  the  hadron number/electron number correlation, depend on the nature of the particle inducing the shower\cite{Stenkin:2002MPLA17}\cite{Stenkin:2009NP196}. 
Thus, the detection of high energy hadrons, addressed to improve the discrimination power in these analysis, is highly advisable. 
A way to deal with this problem avoiding the use of huge and expensive HCALs was brought out in~\cite{Stenkin:2002MPLA17,Stenkin:2001.icrc}. 
In these papers the detection of thermal neutrons generated by EAS hadrons is proposed. 
It is well known that hadrons interacting with ambient matter (air, building, ground, etc.) produce evaporation neutrons due to nuclei disintegration. 
The neutrons have no charge and lose energy only by scattering. 
If the medium is a good moderator, i.e., the absorption cross section is much less than the scattering cross section, the neutrons lose energy via scattering down to the thermal ones (moderation process) and then live in the matter until capture. 
Evaporation neutrons need about 0.5 ms to thermalize in rock (concrete). 
Neutrons are generated abundantly, up to 2 orders of magnitude more than parent hadrons. 
The mean number of evaporation neutrons $<$n$>$ produced by hadrons in a 120 cm layer of surrounding soil (about 3 hadron interaction lengths) and/or construction materials can be estimated using the empirical relationship
\begin{equation}
<n> {\approx} ~36 {\times} E^{0.56}_{h}
\label{nE}
\end{equation}

where $E_h$ is the hadron energy in GeV~\cite{Stenkin:2013CPC37}. 
A large fraction of the evaporation neutrons thermalize, so that recording thermal neutrons can be exploited to reconstruct the hadron content in the shower (Fig. \ref{enda-fig_34}). 
This approach looks very promising for measurements carried out at high altitude. 
Indeed, since the hadron content in EAS increases with the altitude, an abundant production of thermal neutrons  can be predicted for  experiments at 4 (or more) km a.s.l. , about a factor 10 higher than that at sea level~\cite{Stenkin:2013CPC37}. 
These considerations suggested the development of a simple and cheap thermal neutron detector, to be deployed over a large area,  as  'hadron counter' in EAS experiments at mountain level. 
This idea led to the development of the EN-detector, made of a mixture of the well-known inorganic scintillator ZnS(Ag) with $^{6}$LiF, capable of recording both thermal neutrons and charged particles~\cite{Stenkin:2007PAN70}\cite{Stenkin:2008NPS175}.

\begin{figure}[t]
 \centering
 \includegraphics[width=1.0\textwidth]{enda-fig_34}
 \caption{Simulation results: At the same energy, for example, 1PeV, proton has both secondary hadrons $M_h$ and hadron energy $E_h$ and then neutrons $M_n$ about one order higher than ones of Fe~\cite{}Stenkin:2002MPLA17}.}
 \label{enda-fig_34}
 \end{figure}

\subsubsection{Detector Principle}

\begin{figure}[t]
 \centering
 \includegraphics[width=1.0\textwidth]{enda-fig_02}
 \caption{Left: Scheme of the EN-detector. Right top: Photo of the ZnS(Ag)+LiF scintillator used in PRISMA-YBJ. Right bottom: Photo of the ZnS(Ag)+B$_2$O$_3$ scintillator used in LHAASO-ENDA.}
 \label{enda-fig_02}
 \end{figure}

\begin{figure}[t]
 \centering
 \includegraphics[width=1.0\textwidth]{enda-fig_08}
 \caption{Left: pulse shape of noise and neutron. Right: Separation between  noise and neutron in the coordinate system of $Q_{trigger}$ vs $Q_{total}$.}
 \label{shape_ne}
 \end{figure}

\begin{figure}[t]
 \centering
 \includegraphics[width=0.5\textwidth]{enda-4eas_scan_1_run130127-evt932}
 \caption{The shape of the signals from the neutron detectors at PRISMA-YBJ. Upper plot: the pulse from 0 to 2.5 ms. The large peak in the first bin is generated by the EAS electrons. Middle plot: the pulse from 0 to 0.25 ms. Lower plot: the pulse from 0.6 to 0.8 ms (note the different scale on the vertical axis). The small peaks following the first peak are generated by thermal neutrons.}
 \label{easpulse}
 \end{figure}


Of the isotopes used as neutron capture material, $^{3}$He, $^{6}$Li and $^{10}$B are mostly popular. 
The reactions of neutron capture are: \\

$n + ^{3}He \rightarrow  ^{3}H + ^{1}H  + 0.764 MeV  (5333barns)$\\	

$n + ^{6}Li \rightarrow  ^{3}H + ^{4}He + 4.79  MeV	  (940barns)$\\

$n + ^{10}B \rightarrow  ^{7}Li^{*} + ^{4}He \rightarrow ^{7}Li + ^{4}He + 0.48 MeV\gamma + 2.3 MeV (93\%)$ \\
                              \hspace*{4.5cm} $\rightarrow ^{7}Li + ^{4}He + 2.8 MeV (7\%)$ (3980barns)\\

Of the three isotopes, $^{3}$He has the highest cross section of neutron capture, but it is in shortage seriously, not good in timing and not easy to control due to its gaseous state at room temperature. 
$^{6}$Li releases the highest energy during the action, but it is the raw material of nuclear fission so that its purchase is strong limited by government. 
Although capturing neutron with lower released energy than $^{6}$Li, $^{10}$B has larger cross section, and $^{10}$B is much easier to be obtained. 
Moreover, natural Boron contains 19\% versus only 7\% of $^{6}$Li in natural Lithium and this allowed us to make a natural boron compound compatible with lithium ones enriched with $^{6}$Li up to 90\%.

A novel type of ZnS(Ag) scintillator alloyed with B$_{2}$O$_{3}$ with the $^{10}$B isotope about 20\% is developed instead of ZnS(Ag) with $^{6}$LiF. 
Powder of ZnS(Ag) and B$_{2}$O$_{3}$ alloy is not applied on a sheet of plastic or aluminium as convention, but deposited in liquid silicon rubber in the form of a thin one-grain layer. 
The scintillator is not only easier produced in big size, but also transparent for scintillation lights. 
The effective thickness of the scintillator layer is 50 $mg/cm^2$.

The structure of a typical EN-detector is shown in Fig \ref{enda-fig_02}. 
The scintillator of 0.35 $m^2$ area is mounted inside a black cylindrical polyethylene (PE) 200-l tank which is used as the detector housing. 
The scintillator is supported inside the tank to a distance of 30 cm from the photomultiplier (PMT) photocathode. 
A 4$^{''}$-PMT (Beijing Hamamatsu CR-165) is mounted on the tank lid. 
A light reflecting cone made of foiled PE foam of 5-mm thickness is used to improve the light collection. 
As a result, $\sim$ 50 photoelectrons per neutron capture are collected. 
The efficiency for thermal neutron detection in our scintillator was found experimentally by neutron absorption in the scintillator layer to be about 20\%. 
The peculiar characteristics of the EN-detector output, that are weak and fast signals from charged particles compared to high amplitude, slow and delayed signals from thermal neutron capture, make it well suitable for its use in the framework of EAS experiments.

The EN-detector is sensitive to charged particles as well as to thermal neutrons. 
However, because of existence of several time components in this scintillator, the light output is different for different types of particles. 
This characteristic makes possible to select neutron signals from those generated by charged particles (or gamma rays) exploiting their different amplitude and pulse shape. 
Due to the thin layer of the scintillator, charged particles deposit on average only 50 keV against 2.3 - 2.7 MeV deposited during the neutron capture. 
A very high $\alpha$/e ratio, that is the ratio of the light produced by $\alpha$ particles to the light produced by electrons of the same energy, is the main detector feature. 
This feature allows to collect enough light using only one PMT viewing 0.35 $m^2$ scintillator layer. 
The different pulse shape of the neutron signal with respect to the signal produced by charged particles can be fruitfully exploited to remove this background. 
Indeed, slowly moving heavy particles (such as $\alpha$) excite slow components in addition to the emission of fast signals. 
The charge collection time of a signal due to a neutron capture is 10-20 $\mu$s , while the characteristic time of the fast emission induced by charged particles is about 40 ns.  
We compare in Fig. \ref{shape_ne} the pulse shape of the neutron signal with the signal induced by electrons. 
The remarkable difference in shape allows an efficient use of  pulse-shape discrimination to select and record neutron signals in measurements of a neutron flux. 
Note that all signals are digitized with a FADC whose resolution is equal to 1 V / 1024 ch = 1 mV/ch .

The peculiar characteristics of the EN-detector output, that are weak and fast signals from charged particles compared to high amplitude, slow and delayed signals from thermal neutron capture, make it well suitable for its use in the framework of EAS experiments. 
In high energy EAS the time thickness of the shower front is about tens of ns , depending on the distance from the core. 
The individual signals generated by these particles (mainly electrons and positrons) add up to give a signal proportional to their number which can be used also for triggering and timing purposes. 
Delayed signals from thermal neutron capture follow on a time scale of a few milliseconds. 
As an example,we show in Fig. \ref{easpulse} the pulses recorded in a high energy EAS event. 
The first big peak is generated by the large amount of charged particles of the shower front while the  smaller delayed signals are generated by thermal neutrons. 
Thus, the amplitude of the fast signal can be used to measure the charged particle density while the delayed signals measured in a time gate of 10 ms give the number of captured thermal neutrons. 
The selection of electrons and neutrons is automatically performed by the off-line analysis program.

\begin{figure}[t]
 \centering
 \includegraphics[width=1.0\textwidth]{enda-fig_01}
 \caption{Location of ENDA inside LHAASO.}
 \label{enda-fig_01}
 \end{figure}

\begin{figure}[t]
 \centering
 \includegraphics[width=1.0\textwidth]{enda-fig_31}
 \caption{configuration of ENDA-64 (left) and ENDA-400 (right).}
 \label{enda-fig_31}
 \end{figure}


\subsubsection{Progress of ENDA}

 One prototype array of 32 EN-detectors (PRISMA-32) is now running in Moscow~\cite{Stenkin:2011ICRC3}\cite{Gromushkin:2014JInst9}. 
 In order to check the performance of this detector at a high altitude site, a small array composed of four EN-detectors (PRISMA-YBJ) has been installed inside the  hall hosting the ARGO-YBJ experiment at the Yangbajing Cosmic Ray Observatory (Tibet, China, 4300 m a.s.l. , 606 g/cm$^2$).  
 The two arrays operated together, and coincident events have been analyzed to gather information on the PRISMA-YBJ performance~\cite{Bartoli:2016AP81}. 
 After more than 3 years running, PRISMA-YBJ was moved to Tibet University to focus on observation of solar activity and earthquakes. 
 In order to check the performance of the new type EN-detectors at a high altitude site, we built an array of 16 ZnS(Ag) with B$_{2}$O$_{3}$ EN-detectors (LHAASO-ENDA-16) at Tibet University (TU) in Lhasa, Tibet, China (3700 m a.s.l.) In February 2017, and then moved to YBJ at the end of 2018~\cite{Li:2017JINST12}. 
 Up to now, ENDA has totally 66 detectors (ENDA-64 and the other two as backup), ready for deploying  inside LHAASO  to make a hybrid detection of cosmic ray spectrum from 100TeV to 2PeV (Fig. \ref{enda-fig_31} left). 
 After achieving good results, ENDA will be extended to 400 detectors with array area of 10000 $m^2$(Fig. \ref{enda-fig_31} right) , together with LHAASO, to measure energy spectrum at the knee region of iron.

